The Requirement Gatherers' Approach to the 2019 Multi-Agent Programming Contest Scenario

The 2019 Multi-Agent Programming Contest (MAPC) scenario poses many challenges for agents participating in the contest. We discuss The Requirement Gatherers' (TRG) approach to handling the various challenges we faced -- including how we designed our system, how we went about debugging our agents, and the strategy we employed to each of our agents. We conclude the paper with remarks about the performance of our agents, and what we should have done differently.

==> tex/code/container_listing.tex <==
\begin{lstlisting}[language=Java,caption={Using the SPW and Agent containers to log all of the agent's block perceptions}]
// Get the agent container stored by the SPW, agName is the name of the current agent
AgentContainer container = SynchronizedPerceptWatcher
                            .getInstance()
                            .getAgentContainer(agName);

// We only need to iterate through the percepts that are related to the map. There is no casting or hard-coded indices necessary in the internal action to access the information. In this case, we are iterating through the perceived map cells (the Map Percept objects).
container.getAgentMap().getCurrentPercepts().values()
    .forEach(mapPercept -> {
    
        // No casting needed. We check if the current perceived map cell has a block
        if (mapPercept.hasBlock()) {
        
            // We get the block from the Map Percept object, and process it
            Block blockThing = mapPercept.getBlock();
            ts.getLogger().info("Found a block at: " + blockThing.getPosition() + " with type " + blockThing.getDetails());
        }
    });
\end{lstlisting}
